Time Pressure in Software Engineering: A Systematic Review

Large project overruns and overtime work have been reported in the software industry, resulting in additional expense for companies and personal issues for developers. The present work aims to provide an overview of studies related to time pressure in software engineering; specifically, existing definitions, possible causes, and metrics relevant to time pressure were collected, and a mapping of the studies to software processes and approaches was performed. Moreover, we synthesize results of existing quantitative studies on the effects of time pressure on software development, and offer practical takeaways for practitioners and researchers, based on empirical evidence. Our search strategy examined 5,414 sources, found through repository searches and snowballing. Applying inclusion and exclusion criteria resulted in the selection of 102 papers, which made relevant contributions related to time pressure in software engineering. The majority of high quality studies report increased productivity and decreased quality under time pressure. Frequent categories of studies focus on quality assurance, cost estimation, and process simulation. It appears that time pressure is usually caused by errors in cost estimation. The effect of time pressure is most often identified during software quality assurance. The majority of empirical studies report increased productivity under time pressure, while the most cost estimation and process simulation models assume that compressing the schedule increases the total needed hours. We also find evidence of the mediating effect of knowledge on the effects of time pressure, and that tight deadlines impact tasks with an algorithmic nature more severely. Future research should better contextualize quantitative studies to account for the existing conflicting results and to provide an understanding of situations when time pressure is either beneficial or harmful.

==> 1_takeaways.tex <==
IEEE Software

3 points: Improves efficiency and creates a sense of urgency. Reduces  quality, Compromises employee health and equality

TP reduces effectivness and increases efficiency because less time is available / used. How to get best of both worlds. Fake deadlines and buffer times. Or agressive intermediate deadlines as in psyhology experiment

Definitions: Arousal, and the other thing (TODO) Hindrance and something. 

Operationalization: Surveys, Databases (Effort estimates, variations in task complete rates), Affecting computing NLP and using instruments to measure it based measurements


Cause by poor effort estimates, commercial deadlines.
Caused by company culture (prioritize work over everything else)

TP most common in QA phase. Due to internal schedule slippage. 

TP - More willing to report bad news. (Positive). Less communication. 

TP - Reduces quality, SPI willingness, PP, reviews

Buffer time and the time shift perior paper. Different feeling for time. 


Thus, we\todo{If we make the interpretation, shouldn't this be moved outside of this section to somewhere else, e.g. conclusion subsection?} interpret that a central challenge of dealing with time pressure is how to get the benefits of hard work without sacrificing those benefits with short-cutting that then forfeit the benefits of harder work.

type of task effect (DB task, algorithmich defects)

12 patch solutions. 

small proportions of good time pressure. GOOD (personal growt, important challanges to overcome)
high proportions of bad time pressure. DISASTER. (Multi-tasking example of bad, constant task changes. )
